Understanding Underground Incentivized Review Services

While human factors in fraud have been studied by the HCI and security communities, most research has been directed to understanding either the victims' perspectives or prevention strategies, and not on fraudsters, their motivations and operation techniques. Additionally, the focus has been on a narrow set of problems: phishing, spam and bullying. In this work, we seek to understand review fraud on e-commerce platforms through an HCI lens. Through surveys with real fraudsters (N=36 agents and N=38 reviewers), we uncover sophisticated recruitment, execution, and reporting mechanisms fraudsters use to scale their operation while resisting takedown attempts, including the use of AI tools like ChatGPT. We find that countermeasures that crack down on communication channels through which these services operate are effective in combating incentivized reviews. This research sheds light on the complex landscape of incentivized reviews, providing insights into the mechanics of underground services and their resilience to removal efforts.

==> bak/intro_bak_20220729.tex <==
\section{Introduction}
\label{sec:Introduction}

%%Background [importance of review in online marketplaces]


%%Limitations of Prior Art [why existing research on fake reviews is lacking... it's simple to counter? it has been countered]

%%What's new in our problem (as compared to prior art)

%%Proposed Approach [mixed-methods]
%- how both quantitative and qualitative complement each other
%- RQ

%%Key Findings [expanded]

%%Key Contributions

Reviews are an important element in online marketplaces like Amazon, Walmart and eBay. With over a million products and hundreds of options to choose from for every item, customer ratings and reviews play a critical role in a consumer’s decision to buy a product. Stakeholders who profit from a sale (the manufacturer and the seller) naturally have an incentive to obtain as many positive reviews as possible. In recent times, there has been a surge in \textit{third-party sellers} on e-commerce platforms. For example, the Fulfilled By Amazon (FBA)~\footnote{https://sell.amazon.com/fulfillment-by-amazon} program allows third-party sellers to list their products on Amazon. Sellers can manufacture low-quality products at a minimal cost and sell them at a high markup in the US. However, customer reviews and ratings determine the rank of a product; higher ranking products appear on the first page and are shown to more buyers.$82\%$ of adults in the United States check product reviews before buying a product online~\cite{smith2016online}. Studies~\cite{guo2020positive} have shown that positive customer reviews strongly influence a buyer's decision to purchase a new product. This importance of reviews has led to the problem of fake reviews on several popular websites~\cite{mayzlin2014promotional, hu2011fraud, fornaciari2014identifying}. Traditionally, fake reviews were simply opinion spam~\cite{ferrara2019history} where either bots, crowdworkers, or users controlling multiple accounts submitted falsely positive reviews for products. However, of recent, the problem of \textit{incentivized review fraud} is a growing concern.

In this kind of review fraud, sellers give away products at a high discount to buyers in exchange for a positive review. This practice is explicitly banned on Amazon; sellers are not allowed to solicit reviews in exchange for free products. As a workaround, sellers have resorted to creative means; buyers buy the product on Amazon by paying in full, and the seller refunds them via other means outside of Amazon (such as PayPal or gift cards). There exists a vast underground network of sellers, buyers and several intermediaries that facilitates thousands of fake reviews onto Amazon. This can help sellers and their products to bootstrap themselves by gaining sales and reviews for new items.

For products which need bootstrapping in order to promote sales and gain reviews, Amazon offers a program known as the Amazon Vine Program~\footnote{\href{https://www.amazon.com/gp/vine/help}{https://www.amazon.com/gp/vine/help}}. Highly rated reviewers are allowed to select products, get them for free and honestly review them. Sellers, however, prefer to go the underground route; they are guaranteed to get positive, five-star reviews irrespective of how the product is. The seller market is heavily saturated; according to a study~\cite{emon2019amazon}, $50$ new products were uploaded on Amazon every second from Chinese sellers.

In a nutshell, the process works as follows. Through a series of intermediaries (\textit{agents}) who operate via dedicated Facebook groups and targeted advertisements, product sellers reach out to buyers. Agents are contracted by sellers to identify potential buyers who will write a 5-star review in exchange for a full refund of the product. These buyers are referred to as \textit{jennies}. After the buyer receives a product, they write a review, and once a review is live, the seller refunds the buyer via PayPal. Agents receive a commission for every review they help procure. We describe the end-to-end working in greater detail in Section~\ref{sec:end2end}.

Traditionally, fraudulent reviews were generated by bots or through crowdsourcing. However, incentivized reviews are different; the individuals writing the reviews are real humans who are revenue-generating customers for the e-commerce platform. There is a purchase associated with every review, and the incriminating activity that makes the transaction illegal (the refund in exchange for the review) happens outside the e-commerce platform which makes it challenging to detect.

Incentivized fraudulent reviews are a menace to online marketplaces. They mislead buyers, drive down sales for legitimately good products and reduce user trust in the platform. In this paper, we examine the underground reviews economy that deals with reviews and ratings for products on Amazon. Our work aims to study this reviews economy, understand the key players involved, their motivations and incentives, and the tactics they employ to evade detection by Amazon. 

\Paragraph{Research Questions. } We focus on answering the following questions through our research.
\begin{list}{}{}
    \item \textit{\textbf{RQ1.}} Do products which have incentivized reviews exhibit characteristics and trends different than the products which don’t?
    \item \textit{\textbf{RQ2.}} How does the end-to-end process of obtaining a fake 5-star review for a product look like?
    \item \textit{\textbf{RQ3.}} What are the incentives and motivations of the key players involved in the reviews process?
    \item \textit{\textbf{RQ4.}} Incentivized reviews are prohibited on Amazon, and if they flag reviews they are removed. What tactics are used by sellers to evade detection of such reviews?
\end{list}

We apply a \textit{mixed methods} approach to studying the reviews ecosystem and answering our research questions. We scrape and perform statistical analysis on a novel, large dataset. Using qualitative surveys, we investigate the workings of the market, motivations of the key players involved, and evasion tactics.

\Paragraph{Contributions.} We summarize our key contributions~\footnote{All of our collected data, code, and interview transcripts will be made available for further research upon publication of the paper.} as follows:
\begin{itemize}
    \item \textbf{Data.} We construct a gold-standard dataset of $3200$ products and $~400k$ reviews on Amazon that is labelled based on review manipulation. As we compiled this list from posts in the Facebook groups and from products shared by agents, we have high-confidence in our labels. This is the first dataset that has verified ground-truth fraud labels. 
    
    \item \textbf{Statistical Analysis.} We examine the products and reviews for differences in a series of features used traditionally in review spam detection and show that while they are statistically significant, they do not result in high-precision classifiers.
    
    \item \textbf{Audit.} We audit incentivized product detection and removal by Amazon, and find that it is not effective and can easily be countered by sellers by adding more reviews. Out of $1600$ products, Amazon was able to remove only $20$.
    
    \item \textbf{Qualitative Study.} Through interviews with $N = 38$ agents and $N = 36$ buyers we study the reviews ecosystem in depth, analyzing key incentives, procedures and evasion tactics. 
    
\end{itemize}



\remove{
\begin{enumerate}
    \item We construct a dataset of $1600$ products that have incentivized review campaigns running. We also obtain a control set of $1600$ products which are clean (i.e. have no incentivized reviews). We scrape reviews for all these products resulting in $~400k$ reviews. This dataset can be considered gold standard ; we have verified ground truth.
    \item We examine the products and reviews for differences and identify a series of features which help distinguish between incentivized and clean products.
    \item Based on our features, we develop machine learning classifiers.  We devise a two-stage method that first scores aggregate features and then review-level features. Our best classifier operates at an F-1 score of $0.92$.
    \item In order to understand more closely the reviews economy, we conduct a qualitative study by surveying $N = 38$ agents and $N = 37$ buyers involved in the process. Our interviews reveal the economic incentives as well as several tactics used by agents and buyers to evade detection by Amazon. 
\end{enumerate}}

\Paragraph{Key Findings.}
Our results demonstrate the ineffectiveness of existing countermeasures for detecting fraudulent reviews -- even when incentivized reviews are removed, new ones are promptly added back to make up for the removed ones. 
Our qualitative analysis reveals that the incentivized reviews services spans multiple countries, with sellers typically in China, agents in Pakistan and Bangladesh, and buyers in the US, UK, Canada, France, and Germany. 
We find that groups of agents organize jennies using sophisticated training materials, incentive structures, and reporting mechanisms.
Buyers intentionally use evasive tactics such as spreading out the reviews over time and simulating an organic search to circumvent detection. Finally, our investigation revealed that each of the three parties in this ecosystem (sellers, agents and buyers) had incentive to defraud the other two, identifying three kinds of fraud \textit{within} the fraudulent ecosystem.


\Paragraph{Paper Organization.} The rest of the paper is organized as follows. In Section~\ref{sec:RelatedWork}, we provide an overview of the reviews ecosystem, discuss the prior work in this domain and show how our research is different than those. In Section~\ref{sec:Methodology}, we describe our study design and data collection strategies. Then, in Section~\ref{sec:stat_analysis}, we present the statistical tests, machine learning experiments, and online audits that we conducted. Sections~\ref{sec:end2end} and ~\ref{sec:incentives} delve deeper into the reviews market and describe how buyers are recruited and what the incentives for the key players are. Section~\ref{sec:evasion} describes the tactics employed by agents and buyers to evade detection by Amazon. Finally, in section~\ref{sec:conclusion}, we conclude by suggesting countermeasures based on our research.





==> commands.tex <==
\usepackage{enumitem}
\usepackage{subfigure}
\usepackage{amsmath}
\usepackage{euscript}
\usepackage{centernot}
\usepackage{multirow}
%\usepackage{algorithm,algpseudocode}
\usepackage[]{algorithm2e}
% \usepackage{url}
% \PassOptionsToPackage{hyphens}{url}
% \usepackage{hyperref}
\def\UrlBreaks{\do\/\do-\do.\do=\do_\do?\do\&\do\%\do\a\do\b\do\c\do\d\do\e\do\f\do\g\do\h\do\i\do\j\do\k\do\l\do\m\do\n\do\o\do\p\do\q\do\r\do\s\do\t\do\u\do\v\do\w\do\x\do\y\do\z\do\A\do\B\do\C\do\D\do\E\do\F\do\G\do\H\do\I\do\J\do\K\do\L\do\M\do\N\do\O\do\P\do\Q\do\R\do\S\do\T\do\U\do\V\do\W\do\X\do\Y\do\Z\do\0\do\1\do\2\do\3\do\4\do\5\do\6\do\7\do\8\do\9}

% \usepackage{tabularx}

% \newcolumntype{C}{>{\centering\arraybackslash}X}
% % Number of multicolumns      here ↓   and ↓ here (source: https://tex.stackexchange.com/a/236156/134574)
% \newcolumntype{D}{>{\hsize=\dimexpr2\hsize+2\tabcolsep+\arrayrulewidth\relax}C}
\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

%\usetikzlibrary{arrows.meta}
\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{shapes}
\newcommand{\mymkmath}[1]{%
  \tikz[baseline=(char.base)]\node[anchor=south west, draw,rectangle, rounded corners, inner sep=1pt, minimum size=4mm,
    text height=1.5mm](char){\ensuremath{#1}} ;}
\newcommand{\mymk}[1]{%
  \tikz[baseline=(char.base)]\node[anchor=south west, draw,rectangle, rounded corners, inner sep=1pt, minimum size=4mm,
    text height=1.5mm](char){{#1}} ;}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {#1};}}
\newcommand{\Paragraph}[1]{~\vspace*{-0.8\baselineskip}\\{\bf #1}}

\newif\ifshowcomment
%\showcommenttrue
\showcommentfalse

% comment
\ifshowcomment
    \newcommand{\todo}[1]{\textsf{\color{red}{[{TODO: #1}]}}}
    \newcommand{\raj}[1]{\textsf{\color{cyan}{[{Raj: #1}]}}}
    \newcommand{\zubair}[1]{\textsf{\color{purple}{[{Zubair: #1}]}}}

    
\else
    \newcommand{\todo}[1]{}
    \newcommand{\raj}[1]{}
    \newcommand{\highlight}[1]{{\color{black}{#1}}}
    \newcommand{\zubair}[1]{}
\fi

\newcommand{\md}{{{\sf MalDozer}\hspace*{1pt}}}
\newcommand{\dd}{{{\sf DroidDeep}\hspace*{1pt}}}

\newcommand{\remove}[1]{}

